EdgeCentric: Anomaly Detection in Edge-Attributed Networks

Given a network with attributed edges, how can we identify anomalous behavior? Networks with edge attributes are commonplace in the real world. For example, edges in e-commerce networks often indicate how users rated products and services in terms of number of stars, and edges in online social and phonecall networks contain temporal information about when friendships were formed and when users communicated with each other -- in such cases, edge attributes capture information about how the adjacent nodes interact with other entities in the network. In this paper, we aim to utilize exactly this information to discern suspicious from typical node behavior. Our work has a number of notable contributions, including (a) formulation: while most other graph-based anomaly detection works use structural graph connectivity or node information, we focus on the new problem of leveraging edge information, (b) methodology: we introduce EdgeCentric, an intuitive and scalable compression-based approach for detecting edge-attributed graph anomalies, and (c) practicality: we show that EdgeCentric successfully spots numerous such anomalies in several large, edge-attributed real-world graphs, including the Flipkart e-commerce graph with over 3 million product reviews between 1.1 million users and 545 thousand products, where it achieved 0.87 precision over the top 100 results.

==> makefile <==
MAIN=paper
FINAL=final
TEXPARTS= \
	010abstract.tex		\
	020intro.tex		\
	030related.tex		\
	040problem.tex		\
	050method.tex		\
	060results.tex		\
	070discussion.tex	\
	080conclusion.tex	\
	090ack.tex		\
	dfn.tex
BIBFILES= bib/*.bib
FIGFILES= figs/*.png figs/crown/*.png 
ALL= $(MAIN).tex $(BIBFILES) $(FIGFILES) makefile mkfinal.pl

pdf: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)
	pdflatex $(MAIN)
	bibtex $(MAIN)
	pdflatex $(MAIN)
	pdflatex $(MAIN)

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex $(TEXPARTS) mkfinal.pl
	mkfinal.pl $(MAIN).tex > $(FINAL).tex
	dos2unix $(FINAL).tex
	pdflatex $(FINAL)
	bibtex $(FINAL)
	pdflatex $(FINAL)
	pdflatex $(FINAL)


clean:
	\rm -f *.aux *.log *~
	\rm -f *.bbl *.blg
	\rm -f $(FINAL).tex

spotless: clean
	\rm -f $(MAIN).pdf
	\rm -f $(FINAL).pdf

all.tar: $(ALL)
	tar cvf all.tar $(ALL)

